Counseling Summarization using Mental Health Knowledge Guided Utterance Filtering

The psychotherapy intervention technique is a multifaceted conversation between a therapist and a patient. Unlike general clinical discussions, psychotherapy's core components (viz. symptoms) are hard to distinguish, thus becoming a complex problem to summarize later. A structured counseling conversation may contain discussions about symptoms, history of mental health issues, or the discovery of the patient's behavior. It may also contain discussion filler words irrelevant to a clinical summary. We refer to these elements of structured psychotherapy as counseling components. In this paper, the aim is mental health counseling summarization to build upon domain knowledge and to help clinicians quickly glean meaning. We create a new dataset after annotating 12.9K utterances of counseling components and reference summaries for each dialogue. Further, we propose ConSum, a novel counseling-component guided summarization model. ConSum undergoes three independent modules. First, to assess the presence of depressive symptoms, it filters utterances utilizing the Patient Health Questionnaire (PHQ-9), while the second and third modules aim to classify counseling components. At last, we propose a problem-specific Mental Health Information Capture (MHIC) evaluation metric for counseling summaries. Our comparative study shows that we improve on performance and generate cohesive, semantic, and coherent summaries. We comprehensively analyze the generated summaries to investigate the capturing of psychotherapy elements. Human and clinical evaluations on the summary show that ConSum generates quality summary. Further, mental health experts validate the clinical acceptability of the ConSum. Lastly, we discuss the uniqueness in mental health counseling summarization in the real world and show evidences of its deployment on an online application with the support of mpathic.ai

==> Counseling Summarisation -_ Nov Oct21 -_ KDD 22 (1) copy/assets/tables/ChiCCo_Result.tex <==
\begin{table}[t]
\centering
\caption{Results on the clinical conversation ChiCCo dataset. Domain-centric \model\ underperforms in the non-mental health conversation setup. Together with the encouraging performance on \data, it demonstrates the high association of \model\ for the mental health domain.}% for  d atsedue to the absence of  he Unlike mental health counseling conversation dataset, \data, this table shows results obtained on a general clincial conversation dataset, ChiCCo. The results obtained justify the specificity of \model on counseling conversation only.}
\label{tab:chicco}
\vspace{-3mm}
\begin{tabular}{l|rrrrr}\toprule

Model & R-1 & R-2 & R-L & QAE & BS \\
\cmidrule{1-6}

PLM  & $11.82$ & $0.17$ & $14.84$ & $12.37$ & $-1.0890$ \\
RankAE  & $24.00$  & $6.37$ & $20.15$ & $30.25$ & $-0.7466$ \\
SM  & $21.65$ & $7.94$ & $20.37$ & $14.14$ & $-1.001$ \\
% \cdashline{1-6}
Pegasus & $57.54$ & $55.86$ & $27.57$ & $41.10$ & $-0.1253$ \\
T5 &\textbf{71.67} & \textbf{63.62} & \textbf{70.75} & $47.45$ & \textbf{0.2028} \\
\textbf{\model} & $37.13$ & $22.12$ & $17.24$ &\textbf{83.21} & $0.0210$ \\

\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}

% \begin{table}[H]
%     \centering
%     \begin{tabular}{c|c}
%          &  \\
%          & 
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}


==> Counseling Summarisation -_ Nov Oct21 -_ KDD 22 (1) copy/assets/tables/ablation_table.tex <==
\begin{table}[!t]\centering
\caption{Ablation study on the effect of different modules of \model. SH, PD, DF and RT are psychotherapy elements. MH-Know and CCC are knowledge infused module and counseling component classifier module respectively. We present our analysis on five scores to understand all aspects of summary generation.}
\label{tab:ablation_result}
\vspace{-3mm}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|rrrrr}\toprule

% \multirow{2}{*}{Counselling Labels} &\multicolumn{5}{c}{\model\ Generated Summary } \\
% \cmidrule{2-6}

Counselling Label &R-1 &R-2 &R-L &QAE &BS \\
\cmidrule{1-6}

\model\ $-$ SH $-$ PD & $20.92$ & $5.00$ & $7.44$ & $20.71$ & $0.0019$ \\
% \cmidrule{1-6}

\model\ $-$ PD $-$ RT & $36.00$ & $9.00$ & $9.14$ & $20.47$ & $0.2032$ \\
% \cmidrule{1-6}

\model\ $-$ RT $-$ SH & $28.63$ &$8.06$ & $9.55$ & $23.02$ & $-0.0209$ \\
% \cmidrule{1-6}

\model\ $-$ SH & $39.77$ & $9.55$ & $8.98$ & $24.11$ & $0.1908$ \\
% \cmidrule{1-6}

\model\ $-$ PD & $36.87$ & $10.02$ & $11.22$ & \bf 33.38 & $0.2420$ \\
% \cmidrule{1-6}

\model\ $-$ RT & $42.01$ &$9.83$ & $16.50$ & $18.03$ & $0.2060$ \\
% \cmidrule{1-6}

\model\ $-$ MH-Know $-$ CCC & $39.67$ &$9.95$ & $12.69$ & $21.19$ & $0.2003$ \\
% \cmidrule{1-6}

\model\ $-$ MH-Know & $40.42$ &$10.09$ & $11.00$ & $23.97$ & $0.2429$ \\
\cdashline{1-6}
\model\ & \bf 45.36 & \bf 15.71 & \bf 24.75 & 25.42 & \bf 0.3407 \\

% \cmidrule{1-6}
% \model\ - PD &31.44 &5.63 & 27.38 &33.55 & -0.5655 \\\cmidrule{1-6}


% RankAE \cite{Zou_Lin_Zhao_Kang_Jiang_Sun_Zhang_Huang_Liu_2021} & 25.57 & 3.43 & 24.16 & 29.98 & -1.0631  & 24  & 6.37 & 20.15 & 30.25 & -0.7466 \\\cmidrule{1-11}

% \textbf{\model} &\textbf{45.36} &\textbf{15.71} & 24.75 & 25.42 &\textbf{0.3407} & 7.13 & 22.12 & 17.24 &\textbf{83.21} & 0.0284 \\\midrule

\bottomrule
\end{tabular}}
\vspace{-7mm}
\end{table}

==> Counseling Summarisation -_ Nov Oct21 -_ KDD 22 (1) copy/assets/tables/concise_summary_feature.tex <==
% \begin{table}
% \centering
% \fontsize{6}{7}\selectfont
% % \resizebox{220}{!}{%
% \begin{tabular}{c|p{28em}} \toprule
% \textbf{Model} & {\centering \textbf{Summaries}} \\\cmidrule{1-2}
% T5 & \vspace{-1.5mm}{\em Patient is asked a series of questions to test their housing. Patients {\color{green!50!black}do not want to take drugs}, police arrest them and others in their area. {\color{brown!60!black}They secretly talk about the incident}. The patient lives with friends from different places including the city, where they are arrested or taken into custody. The patients feel they have no medical condition such as diabetes or stroke. {\color{brown!60!black}These occured recently}. The patient has had problems with housing due {\color{red!70!black}augensis}. Patients feel {\color{cyan!50!black}they have been victimized by drug abusers since they were 12 years old}. They know {\color{red!70!black}people who don't use marijuana to steal}}\\ \cdashline{1-2}\\
% \model & \vspace{-2.5mm}{\em Whenever there is a basketball or or football, the patient does not really hear what to take. {\color{green!50!black}Patient feels overwhelming} and {\color{cyan!50!black}feels like having this issue since childhood}. Therapist made him realise his problems and patient was curing gradually. Therapist suggested him use. {\color{brown!60!black}The patient was raised Catholic and they feel guilty about spending more money on drugs and parties}. The patient has switched 12 houses in the past year and feel it must have affected their kids. The patient occasionally borrows money and gets less sleep in general}\\\cmidrule{1-2}
% T5 & \vspace{-1.5mm}{\em {\color{brown!60!black}The patient is tired when they have to go to work and it's a bit frustrating for them}. They feel tired throughout the day without any food, no panic attacks, no medical condition such as diabetes or stroke. Patients are in a position where they {\color{red!70!black}can} {\color{green!50!black}focus on anything}. They do not want pills to reduce stress hence their life is limited by diet. The patient has lost three pounds in recent weeks due to this fatigue}\\ \cdashline{1-2}\\
% \model & \vspace{-2.5mm}{\em Whenever the patient goes to work. {\color{green!50!black}The patient is worried that they might have ADHD}. The patient does not suffer from depression, anxiety nor use drugs or call it a metaphysical stuff. The patient wishes to get better and needs something to hold. The patient feel they sway at things, and they have two options. The patient was sent in by a counselor fearing they might hurt themselves. {\color{cyan!50!black}The patient's dad had committed suicide 15 years ago and their sister had attempted once}. {\color{green!50!black}The patient has been diagnosed with depression and anxiety}. {\color{brown!60!black}The patient lives alone}}\\
% \bottomrule
% \end{tabular}
% % }
% \caption{Comparative analysis on generated summaries between T5 and \model\ model. {\color{green!50!black}Green} denotes primary medical condition information, {\color{cyan!50!black}Cyan} denotes SR information, {\color{brown!60!black}{Brown}} denotes RT information and {\color{red!70!black}Red} denotes errors/irrelevance in generated summaries. Side-by-Side comparison shows the contextual information captured in $\model$ which is lacking in T5's outputs.}
% \label{tab:con_sum_features}
% \vspace{-5mm}
% \end{table}

\begin{table*}
\centering
\caption{Comparative analysis on generated summaries between T5 and \model\ model. {\color{green!50!black}Green} denotes primary medical condition information, {\color{cyan!50!black}Cyan} denotes SH information, {\color{brown!60!black}{Brown}} denotes RT information and {\color{red!70!black}Red} denotes errors/irrelevance in generated summaries. Comparison shows $\model$ captures better contextual information compared to T5.}
\label{tab:con_sum_features}
\vspace{-3mm}
% \fontsize{6}{7}\selectfont
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|p{58em}} \toprule
\textbf{Model} & {\centering \textbf{Summaries}} \\\cmidrule{1-2}
T5 & {\em Patient is asked a series of questions to test their housing. Patients {\color{green!50!black}do not want to take drugs}, police arrest them and others in their area. {\color{brown!60!black}They secretly talk about the incident}. The patient lives with friends from different places including the city, where they are arrested or taken into custody. The patients feel they have no medical condition such as diabetes or stroke. {\color{brown!60!black}These occured recently}. The patient has had problems with housing due {\color{red!70!black}augensis}. Patients feel {\color{cyan!50!black}they have been victimized by drug abusers since they were 12 years old}. They know {\color{red!70!black}people who don't use marijuana to steal}}\\ \cdashline{1-2}

\model & {\em Whenever there is a basketball or or football, the patient does not really hear what to take. {\color{green!50!black}Patient feels overwhelming} and {\color{cyan!50!black}feels like having this issue since childhood}. Therapist made him realise his problems and patient was curing gradually. Therapist suggested him use. {\color{brown!60!black}The patient was raised Catholic and they feel guilty about spending more money on drugs and parties}. The patient has switched 12 houses in the past year and feel it must have affected their kids. The patient occasionally borrows money and gets less sleep in general}\\ \hline

T5 & \textit{{\color{brown!60!black}The patient is tired when they have to go to work and it's a bit frustrating for them}. They feel tired throughout the day without any food, no panic attacks, no medical condition such as diabetes or stroke. Patients are in a position where they {\color{red!70!black}can} {\color{green!50!black}focus on anything}. They do not want pills to reduce stress hence their life is limited by diet. The patient has lost three pounds in recent weeks due to this fatigue} \\
 \cdashline{1-2}

\model & {\em Whenever the patient goes to work. {\color{green!50!black}The patient is worried that they might have ADHD}. The patient does not suffer from depression, anxiety nor use drugs or call it a metaphysical stuff. The patient wishes to get better and needs something to hold. The patient feel they sway at things, and they have two options. The patient was sent in by a counselor fearing they might hurt themselves. {\color{cyan!50!black}The patient's dad had committed suicide 15 years ago and their sister had attempted once}. {\color{green!50!black}The patient has been diagnosed with depression and anxiety}. {\color{brown!60!black}The patient lives alone}}\\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table*}



==> Counseling Summarisation -_ Nov Oct21 -_ KDD 22 (1) copy/assets/tables/dataset_stats.tex <==
\begin{table}[t]
    \centering
    \caption{Distribution of psychotherapy elements  in \data\ dataset. Here, \textbf{\#D:} Number of dialogues; \textbf{\#U:} Number of utterances; \textbf{U/D:} Utterances per dialogue; \textbf{Sp:} speaker; \textbf{Th:} Therapist; and \textbf{Pt:}. Patient. The train, test, and validation splits are 70:20:10.}
    \label{tab:counts}
    \vspace{-3mm}
    % \begin{adjustbox}{width=1\textwidth}
    \resizebox{1\columnwidth}{!}
    {
    % \small
    \begin{tabular}{c c c c c c c c c c c c c c c c}
    % \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule[1pt]
         &  &  &  &  & \multicolumn{6}{c}{\bf Counseling Components} & \\ 
         \cline{6-11}
         &  &  & \multicolumn{2}{c}{\bf Discussion Filler} & \multicolumn{2}{c}{\bf SH} & \multicolumn{2}{c}{\bf RT} & \multicolumn{2}{c}{\bf PD}\\ 
         \cline{4-11}
        \textbf{Split} & \textbf{\#D} & \textbf{Sp.} & U/D & \#U & U/D & \#U & U/D & \#U & U/D & \#U & \textbf{Total} \\
        \toprule[1pt]
        \multirow{2}{*}{\textbf{Train}} & \multirow{2}{*}{152} & Pt & $5.02$ & $764$ & $5.67$ & $862$ & $2.52$ & $383$ & $18.84$ & $2863$ & $4766$\\
         & & Th & $8.10$ & $1232$ & $8.17$ & $1243$ & $4.22$ & $642$ & $10.80$ & $1643$ & $4877$\\
        \cdashline{1-12} 
        \multirow{2}{*}{\textbf{Test}} & \multirow{2}{*}{39} & Pt & $3.43$ & $134$ & $2.95$ & $115$ & $1.00$ & $39$ & $18.38$ & $717$ & $1004$\\
         & & Th & $5.46$ & $213$ & $4.51$ & $176$ & $4.43$ & $173$ & $11.28$ & $440$ & $1006$\\
        \cdashline{1-12}
        \multirow{2}{*}{\textbf{Val}} & \multirow{2}{*}{21} & Pt & $8.09$ & $170$ & $4.23$ & $89$ & $2.28$ & $48$ & $13.80$ & $290$ & $594$\\
         & & Th & $10.48$ & $220$ & $5.57$ & $117$ & $4.66$ & $98$ & $7.38$ & $155$ & $597$\\ \cline{1-12}
         \multirow{2}{*}{\textbf{Total}} & \multirow{2}{*}{212} & Pt & $5.51$ & $1068$ & $4.28$ & $1066$ & $1.60$ & $470$ & $17.00$ & $3870$ & $6364$\\
         & & Th & $8.01$ & $1665$ & $6.08$ & $1536$ & $4.44$ & $913$ & $9.82$ & $2238$ & $6480$\\ 
         \toprule[1pt]
        %  \multicolumn{15}{c}{} \\

    \end{tabular}}
    % \end{adjustbox}

    \vspace{-5mm}
\end{table}

==> Counseling Summarisation -_ Nov Oct21 -_ KDD 22 (1) copy/assets/tables/human_eval.tex <==
\begin{table}[!t]
\centering
\caption{Human evaluation on the summaries generated from \model\ model.}\label{tab:humaneval}
 \vspace{-3mm}
\begin{tabular}{l|cccc}\toprule
Model & Relevance & Consistency & Fluency & Coherence \\
\cmidrule{1-5}
RankAE  & 2.80 & 2.91 & 3.02 & 2.98\\
T5  &2.99& 3.05& 3.04& 2.95\\
\cdashline{1-5}
\textbf{\model} & 3.37 & 3.22 & 3.11 & 3.13\\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}

==> Counseling Summarisation -_ Nov Oct21 -_ KDD 22 (1) copy/assets/tables/mental_health_rating_aspects.tex <==
\begin{table*}[ht!]
\centering
\begin{tabular}{|c|p{20em}|p{20em}|}\hline
Construct & Definition & Application\\
\hline
Affective attitude & How an individual feels about an intervention & What are your perceptions of the intervention based upon your clinical knowledge\\
\hline
Burden & Perceived amount of effort required to participate & How much effort is required to understand the intervention, consider: spelling, grammar, overall interpretation\\
\hline
Ethicality & Extent to which this is a good fit with your organizations' value system & How does this align with your respective code of ethics? Are there concerns?\\
\hline
Intervention Coherence & Extent to which the intervention is understood & How well the summaries are understood\\
\hline
Opportunity Cost & The extent to which one would benefit from using this intervention & Pros and cons of using this intervention in your respective setting\\
\hline
Perceived Effectiveness & Extent to whcih this intervention will perform in the intended setting & How well this will perform in your clinical setting\\
\hline
\end{tabular}
\caption{Individual metrics as reported in Table \ref{tab:rater_eval} are explained with the application setting.}
% \vspace{-5mm}
\label{tab:mental_health_aspects}
\end{table*}

==> Counseling Summarisation -_ Nov Oct21 -_ KDD 22 (1) copy/assets/tables/rater_evaluation.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l|cccccc}\toprule
Rater & Affective Attitude & Burden & Ethicality & Intervention Coherence & Opportunity Cost & Perceived Effectiveness\\
\hline
Rater-1  & 0.875 & 1 & 1 & 1.125 & 0.875 & 0.875\\
Rater-2  & 0.75 & 0.875 & 1 & 0.875 & 0.875 & 1\\
\cdashline{1-7}
\textbf{Average} & 0.813 & 0.936 & 1 & 1 & 0.875 & 0.936\\
\bottomrule
\end{tabular}
\caption{Mental health experts rate the summaries generated by \model\  on mental-health aspects.}
\vspace{-5mm}
\label{tab:rater_eval}
\end{table*}

==> Counseling Summarisation -_ Nov Oct21 -_ KDD 22 (1) copy/assets/tables/summary_dialogue_comparison.tex <==
\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{||c|c|c|c|c|c|c||} 
\hline
Summary & \multicolumn{3}{c|}{Generated} & \multicolumn{3}{c|}{Golden} \\\cline{2-7}
& Rec. & Prec. &  F1 & Rec. & Prec. & F1\\
\hline
w/o chit-chat & 72.21 & 7.46 & 13.16 & 50.24 & 4.90 & 8.46\\ 
\hline
w/o chit-chat/PD & 60.60 & 10.75 & 16.80 & 40.59 & 6.48 & 10.14\\ 
\hline
with SR & 41.32 & 16.25 & 21.07 & 27.26 & 9.67 & 12.77\\ 
\hline
with chit-chat & 9.14 & 6.64 & 7.15 & 7.93 & 5.26 & 5.47\\ 
\hline
with PD & 51.63 & 8.54 & 13.80 & 39.24 & 6.02 & 9.65\\ 
\hline
with RT & 41.62 & 8.18 & 12.98 & 31.26 & 5.77 & 9.04\\ 
\hline
\end{tabular}
}
\caption{Experimental results to show counselling information capture (label wise unigram overlap) from generated/golden summaries and dialogue utterances. Each row denotes utterances concatenated with/without certain sub-topics.}
\label{tab:sum_comparison}
\end{table}

==> Counseling Summarisation -_ Nov Oct21 -_ KDD 22 (1) copy/assets/tables/summary_feature_capture.tex <==
\begin{table*}[ht!]
    \centering
    \fontsize{2}{3.5}\selectfont
    % \begin{adjustbox}{width=1\textwidth}
    \resizebox{\textwidth}{!}
    {
    % \small
    \begin{tabular}{|p{28em}|p{28em}|}
    % \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule[1pt]
         \multicolumn{1}{c}{\bf T5 Summary} & \multicolumn{1}{c}{\bf \model Summary}\\ 
         \hline\hline
         {\em {\color{brown}Patient is asked a series of questions} to test their housing. Patients {\color{green}do not want to take drugs}, police arrest them and others in their area. {\color{red}They secretly talk about the incident}. The patient lives with friends from different places including the city, where they are arrested or taken into custody. The patients feel they have no medical condition such as diabetes or stroke. {\color{brown}These occured recently}. The patient has had problems with housing due {\color{red}augensis}. Patients feel {\color{cyan}they have been victimized by drug abusers since they were 12 years old}. They know {\color{red}people who don't use marijuana to steal}} & {\em When there is a basketball or or football. The patient does not really hear what to take. {\color{green}Patient feels overwhelming} and {\color{cyan}feels like having this issue since childhood}. Therapist made him realise his problems and patient was curing gradually. Therapist suggested him use. {\color{brown}The patient was raised Catholic and they feel guilty about spending more money on drugs and parties}. The patient has switched 12 houses in the past year and feel it must have affected their kids. The patient occasionally borrows money and gets less sleep in general}\\
         \hline
         {\em {\color{brown}The patient is tired when they have to go to work and it's a bit frustrating for them}. They feel tired throughout the day without any food, no panic attacks, no medical condition such as diabetes or stroke. Patients are in a position where they {\color{red}can} {\color{green}focus on anything}. They do not want pills to reduce stress hence their life is limited by diet. The patient has lost three pounds in recent weeks due to this fatigue} & {\em Whenever the patient goes to work. {\color{green}The patient is worried that they might have ADHD}. The patient does not suffer from depression, anxiety nor use drugs or call it a metaphysical stuff. The patient wishes to get better and needs something to hold. The patient feel they sway at things, and they have two options. The patient was sent in by a counselor fearing they might hurt themselves. {\color{cyan}The patient's dad had committed suicide 15 years ago and their sister had attempted once}. {\color{green}The patient has been diagnosed with depression and anxiety}. {\color{brown}The patient lives alone}}\\
         \hline
         {\em {\color{red}The patient is diagnosed of cancer}. They have scars when they cut themselves with a razor. The patient has the same arm as always on their wrist. The patient has deep pockets and no surgical condition. {\color{red}The patient does not want to lose sight of the patient}. The patient has been experiencing this since high school. They have had scars in the past few years. The patient used to cut down on a razor but instead of {\color{green}using marijuana}, it helps them to reduce anxiety. In another instance when the {\color{red}Patient was diagnosed for which the patient is diagnosed (or depression)}} & {\em {\color{red}Whenever whenever whenever} There is a lot of marijuana, where they even forgot to look. The Patient visits therapist for feeling and {\color{green}couldn't get back on track}. Therapist knew that patient had such feelings in the past but this time patient found harder. Two months ago patient visited GP after that GP {\color{red}reffered} to therapist} \\
         
 \toprule[1pt]
    \end{tabular}}
    % \end{adjustbox}

    \caption{Comparative analysis on generated summaries between T5 and \model model. {\color{green}Green} denotes primary medical condition information, {\color{cyan}Cyan} denotes SR information, {\color{brown}{Brown}} denotes RT information and {\color{red}Red} denotes errors/irrelevance in generated summaries. Side-by-Side comparison shows the contextual information captured in \model which is lacking in T5's outputs.}
    \label{tab:error:summaries}
\end{table*}

==> Counseling Summarisation -_ Nov Oct21 -_ KDD 22 (1) copy/assets/tables/summary_results_combined.tex <==

\begin{table}[!t]\centering
%\resizebox{\columnwidth}{!}{
\begin{tabular}{l|rrrrr}\toprule
% \multirow{2}{*}{Models} &\multicolumn{5}{c}{Result on \data } \\
% \cmidrule{2-6}
Model &R-1 &R-2 &R-L &QAE &BS \\
\cmidrule{1-6}
\multicolumn{6}{c}{Baselines}\\
\hline

SM  & 20.46 & 3.80 & 18.87 & 20.22 & -0.94 \\
T5 &31.44 &5.63 & 27.38 &33.55 & -0.56\\
Pegasus & 29.71 & 7.77 & 27.57 &\textbf{36.80} & -0.61\\
RankAE  & 25.57 & 3.43 & 24.16 & 29.98 & -1.06\\
PLM  &34.24 & 11.19 &\textbf{33.35} & 24.34 & -0.86\\
\cdashline{1-6}
\textbf{\model} &\textbf{45.36} &\textbf{15.71} & 24.75 & 25.42 &\textbf{0.34} \\

\hline
\multicolumn{6}{c}{Ablation Study}\\
\hline

\model\ $-$ SH $-$ PD & $20.92$ & $5.00$ & $7.44$ & $20.71$ & $0.0019$ \\
% \cmidrule{1-6}

\model\ $-$ PD $-$ RT & $36.00$ & $9.00$ & $9.14$ & $20.47$ & $0.2032$ \\
% \cmidrule{1-6}

\model\ $-$ RT $-$ SH & $28.63$ &$8.06$ & $9.55$ & $23.02$ & $-0.0209$ \\
% \cmidrule{1-6}

\model\ $-$ SH & $39.77$ & $9.55$ & $8.98$ & $24.11$ & $0.1908$ \\
% \cmidrule{1-6}

\model\ $-$ PD & $36.87$ & $10.02$ & $11.22$ & $33.38$ & $0.2420$ \\
% \cmidrule{1-6}

\model\ $-$ RT & $42.01$ &$9.83$ & $16.50$ & $18.03$ & $0.2060$ \\
% \cmidrule{1-6}

\model\ $+$ DF & $39.67$ &$9.95$ & $12.69$ & $21.19$ & $0.2003$ \\
% \cmidrule{1-6}

\model\ $-$ MH-Know & $40.42$ &$10.09$ & $11.00$ & $23.97$ & $0.2429$ \\
\cdashline{1-6}
\model\ & $45.36$ & $15.71$ & $24.75$ & $25.42$ & $0.3407$ \\

\bottomrule
\end{tabular}
\caption{In the upper section of the table, we present the baseline results obtained on \data. We report  Rouge-1 (R-1), Rouge-2 (R-2), Rouge-L (R-L), Bleurt Score (BS) and QuestEval Score (QAE). In the lower section of the table, we show ablation study studying the effect of psychotherapy elements SH, PD, DF, and RT. 
% \hl{table 2 and ablation table could be merged}% Our model, \model\ yields better Rouge scores than competing baselines on R-1, R-2 and BS. We also presented a problem-specific metric, MHIC in Section \ref{mhic}.
}
%\vspace{-5mm}
\label{tab:result_and_ablation}
\end{table}


% \begin{table}[!t]\centering
% %\resizebox{\columnwidth}{!}{
% \begin{tabular}{l|rrrrr}\toprule

% % \multirow{2}{*}{Counselling Labels} &\multicolumn{5}{c}{\model\ Generated Summary } \\
% % \cmidrule{2-6}

% Counselling Label &R-1 &R-2 &R-L &QAE &BS \\
% \cmidrule{1-6}

% \model\ $-$ SH $-$ PD & $20.92$ & $5.00$ & $7.44$ & $20.71$ & $0.0019$ \\
% % \cmidrule{1-6}

% \model\ $-$ PD $-$ RT & $36.00$ & $9.00$ & $9.14$ & $20.47$ & $0.2032$ \\
% % \cmidrule{1-6}

% \model\ $-$ RT $-$ SH & $28.63$ &$8.06$ & $9.55$ & $23.02$ & $-0.0209$ \\
% % \cmidrule{1-6}

% \model\ $-$ SH & $39.77$ & $9.55$ & $8.98$ & $24.11$ & $0.1908$ \\
% % \cmidrule{1-6}

% \model\ $-$ PD & $36.87$ & $10.02$ & $11.22$ & $33.38$ & $0.2420$ \\
% % \cmidrule{1-6}

% \model\ $-$ RT & $42.01$ &$9.83$ & $16.50$ & $18.03$ & $0.2060$ \\
% % \cmidrule{1-6}

% \model\ $+$ DF & $39.67$ &$9.95$ & $12.69$ & $21.19$ & $0.2003$ \\
% % \cmidrule{1-6}

% \model\ $-$ MH-Know & $40.42$ &$10.09$ & $11.00$ & $23.97$ & $0.2429$ \\
% \cdashline{1-6}
% \model\ & $45.36$ & $15.71$ & $24.75$ & $25.42$ & $0.3407$ \\

% % \cmidrule{1-6}
% % \model\ - PD &31.44 &5.63 & 27.38 &33.55 & -0.5655 \\\cmidrule{1-6}


% % RankAE \cite{Zou_Lin_Zhao_Kang_Jiang_Sun_Zhang_Huang_Liu_2021} & 25.57 & 3.43 & 24.16 & 29.98 & -1.0631  & 24  & 6.37 & 20.15 & 30.25 & -0.7466 \\\cmidrule{1-11}

% % \textbf{\model} &\textbf{45.36} &\textbf{15.71} & 24.75 & 25.42 &\textbf{0.3407} & 7.13 & 22.12 & 17.24 &\textbf{83.21} & 0.0284 \\\midrule

% \bottomrule
% \end{tabular}
% \caption{Ablation study on the effect of different modules of \model. SH, PD, DF and RT are therapy constituents. We present our analysis on five scores to understand all aspects of summary generation.}
% \label{tab:ablation_result}
% \vspace{0mm}
% \end{table}

==> Counseling Summarisation -_ Nov Oct21 -_ KDD 22 (1) copy/assets/tables/two_data_result.tex <==
% \begin{table}[!t]\centering
% % \scalebox{1.1}
% \resizebox{\columnwidth}{!}{
% % \scriptsize

% \begin{tabular}{l|rrrrr|rrrrrr}\toprule

% \multirow{2}{*}{System} &\multicolumn{5}{c|}{HOPESUM} &\multicolumn{5}{c}{ChiCCo} \\\cmidrule{2-11}

% &R-1 &R-2 &R-L & QAE &BS  &R-1 &R-2 &R-L &QAE & BS \\
% \cmidrule{1-11}

% SM  & 20.46 & 3.80 & 18.87 & 20.22 & -0.94  & 21.65 & 7.94 & 20.37 & 14.14 & -1.0 \\
% % \cmidrule{1-11}

% T5 &31.44 &5.63 & 27.38 &33.55 & -0.56  &\textbf{71.67} & \textbf{63.62} & \textbf{70.75} & 47.45 & \textbf{0.20} \\
% % \cmidrule{1-11}

% Pegasus & 29.71 & 7.77 & 27.57 &\textbf{36.80} & -0.61 &   
% % \cmidrule{1-11}

% RankAE  & 25.57 & 3.43 & 24.16 & 29.98 & -1.06  & 24.00  & 6.37 & 20.15 & 30.25 & -0.74 \\
% % \cmidrule{1-11}


% PLM  &34.24 & 11.19 &\textbf{33.35} & 24.34 & -0.86  &11.82 & 0.17 & 14.84 & 12.37 & -1.08 \\
% % \cmidrule{1-11}

% \textbf{\model} &\textbf{45.36} &\textbf{15.71} & 24.75 & 25.42 &\textbf{0.34} & 7.13 & 22.12 & 17.24 &\textbf{83.21} & 0.02 \\
% % \midrule

% \bottomrule
% \end{tabular}}
% \caption{Comparative analysis on two datasets -- HOPESUM and ChiCCo. We report  Rouge-1 (R-1), Rouge-2 (R-2), and Rouge-L (R-L) scores for five abstractive baselines. Our model, \model\ yields better Rouge scores than competing baselines. We also compare the methods based on Bleurt Score (BS) and QuestEval Score (QAE). We observe that we perform better with R-1, R-2, BS. We also presented a problem-specific metric, MHIC in Section \ref{mhic}.}
% \label{tab:main_result}
% \vspace{-5mm}
% \end{table}


% --------------

\begin{table}[!t]\centering
\caption{Results obtained on \data. We report  Rouge-1 (R-1), Rouge-2 (R-2), Rouge-L (R-L), Bleurt Score (BS) and QuestEval Score (QAE).}\label{tab:baselines}
\vspace{-3mm}
%\resizebox{\columnwidth}{!}{
\begin{tabular}{l|rrrrr}\toprule
% \multirow{2}{*}{Models} &\multicolumn{5}{c}{Result on \data } \\
% \cmidrule{2-6}
Model &R-1 &R-2 &R-L &QAE &BS \\
\cmidrule{1-6}

PLM  &34.24 & 11.19 &\textbf{33.35} & 24.34 & -0.8678\\
RankAE  & 25.57 & 3.43 & 24.16 & 29.98 & -1.063\\
SM  & 20.46 & 3.80 & 18.87 & 20.22 & -0.9454 \\
Pegasus & 29.71 & 7.77 & 27.57 &\textbf{36.80} & -0.6130\\
T5 &31.44 &5.63 & 27.38 &33.55 & -0.5655\\
\cdashline{1-6}
\textbf{\model} &\textbf{45.36} &\textbf{15.71} & 24.75 & 25.42 &\textbf{0.3407} \\

\bottomrule
\end{tabular}
\vspace{-3mm}
\end{table}


==> assets/tables/summary_dialogue_comparison.tex <==
\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{||c|c|c|c|c|c|c||} 
\hline
Summary & \multicolumn{3}{c|}{Generated} & \multicolumn{3}{c|}{Golden} \\\cline{2-7}
& Rec. & Prec. &  F1 & Rec. & Prec. & F1\\
\hline
w/o chit-chat & 72.21 & 7.46 & 13.16 & 50.24 & 4.90 & 8.46\\ 
\hline
w/o chit-chat/PD & 60.60 & 10.75 & 16.80 & 40.59 & 6.48 & 10.14\\ 
\hline
with SR & 41.32 & 16.25 & 21.07 & 27.26 & 9.67 & 12.77\\ 
\hline
with chit-chat & 9.14 & 6.64 & 7.15 & 7.93 & 5.26 & 5.47\\ 
\hline
with PD & 51.63 & 8.54 & 13.80 & 39.24 & 6.02 & 9.65\\ 
\hline
with RT & 41.62 & 8.18 & 12.98 & 31.26 & 5.77 & 9.04\\ 
\hline
\end{tabular}
}
\caption{Experimental results to show counselling information capture (label wise unigram overlap) from generated/golden summaries and dialogue utterances. Each row denotes utterances concatenated with/without certain sub-topics.}
\label{tab:sum_comparison}
\end{table}

==> assets/tables/summary_feature_capture.tex <==
\begin{table*}[ht!]
    \centering
    \fontsize{2}{3.5}\selectfont
    % \begin{adjustbox}{width=1\textwidth}
    \resizebox{\textwidth}{!}
    {
    % \small
    \begin{tabular}{|p{28em}|p{28em}|}
    % \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule[1pt]
         \multicolumn{1}{c}{\bf T5 Summary} & \multicolumn{1}{c}{\bf \model Summary}\\ 
         \hline\hline
         {\em {\color{brown}Patient is asked a series of questions} to test their housing. Patients {\color{green}do not want to take drugs}, police arrest them and others in their area. {\color{red}They secretly talk about the incident}. The patient lives with friends from different places including the city, where they are arrested or taken into custody. The patients feel they have no medical condition such as diabetes or stroke. {\color{brown}These occured recently}. The patient has had problems with housing due {\color{red}augensis}. Patients feel {\color{cyan}they have been victimized by drug abusers since they were 12 years old}. They know {\color{red}people who don't use marijuana to steal}} & {\em When there is a basketball or or football. The patient does not really hear what to take. {\color{green}Patient feels overwhelming} and {\color{cyan}feels like having this issue since childhood}. Therapist made him realise his problems and patient was curing gradually. Therapist suggested him use. {\color{brown}The patient was raised Catholic and they feel guilty about spending more money on drugs and parties}. The patient has switched 12 houses in the past year and feel it must have affected their kids. The patient occasionally borrows money and gets less sleep in general}\\
         \hline
         {\em {\color{brown}The patient is tired when they have to go to work and it's a bit frustrating for them}. They feel tired throughout the day without any food, no panic attacks, no medical condition such as diabetes or stroke. Patients are in a position where they {\color{red}can} {\color{green}focus on anything}. They do not want pills to reduce stress hence their life is limited by diet. The patient has lost three pounds in recent weeks due to this fatigue} & {\em Whenever the patient goes to work. {\color{green}The patient is worried that they might have ADHD}. The patient does not suffer from depression, anxiety nor use drugs or call it a metaphysical stuff. The patient wishes to get better and needs something to hold. The patient feel they sway at things, and they have two options. The patient was sent in by a counselor fearing they might hurt themselves. {\color{cyan}The patient's dad had committed suicide 15 years ago and their sister had attempted once}. {\color{green}The patient has been diagnosed with depression and anxiety}. {\color{brown}The patient lives alone}}\\
         \hline
         {\em {\color{red}The patient is diagnosed of cancer}. They have scars when they cut themselves with a razor. The patient has the same arm as always on their wrist. The patient has deep pockets and no surgical condition. {\color{red}The patient does not want to lose sight of the patient}. The patient has been experiencing this since high school. They have had scars in the past few years. The patient used to cut down on a razor but instead of {\color{green}using marijuana}, it helps them to reduce anxiety. In another instance when the {\color{red}Patient was diagnosed for which the patient is diagnosed (or depression)}} & {\em {\color{red}Whenever whenever whenever} There is a lot of marijuana, where they even forgot to look. The Patient visits therapist for feeling and {\color{green}couldn't get back on track}. Therapist knew that patient had such feelings in the past but this time patient found harder. Two months ago patient visited GP after that GP {\color{red}reffered} to therapist} \\
         
 \toprule[1pt]
    \end{tabular}}
    % \end{adjustbox}

    \caption{Comparative analysis on generated summaries between T5 and \model model. {\color{green}Green} denotes primary medical condition information, {\color{cyan}Cyan} denotes SR information, {\color{brown}{Brown}} denotes RT information and {\color{red}Red} denotes errors/irrelevance in generated summaries. Side-by-Side comparison shows the contextual information captured in \model which is lacking in T5's outputs.}
    \label{tab:error:summaries}
\end{table*}

==> assets/tables/summary_results_combined.tex <==

\begin{table}[!t]\centering
%\resizebox{\columnwidth}{!}{
\begin{tabular}{l|rrrrr}\toprule
% \multirow{2}{*}{Models} &\multicolumn{5}{c}{Result on \data } \\
% \cmidrule{2-6}
Model &R-1 &R-2 &R-L &QAE &BS \\
\cmidrule{1-6}
\multicolumn{6}{c}{Baselines}\\
\hline

SM  & 20.46 & 3.80 & 18.87 & 20.22 & -0.94 \\
T5 &31.44 &5.63 & 27.38 &33.55 & -0.56\\
Pegasus & 29.71 & 7.77 & 27.57 &\textbf{36.80} & -0.61\\
RankAE  & 25.57 & 3.43 & 24.16 & 29.98 & -1.06\\
PLM  &34.24 & 11.19 &\textbf{33.35} & 24.34 & -0.86\\
\cdashline{1-6}
\textbf{\model} &\textbf{45.36} &\textbf{15.71} & 24.75 & 25.42 &\textbf{0.34} \\

\hline
\multicolumn{6}{c}{Ablation Study}\\
\hline

\model\ $-$ SH $-$ PD & $20.92$ & $5.00$ & $7.44$ & $20.71$ & $0.0019$ \\
% \cmidrule{1-6}

\model\ $-$ PD $-$ RT & $36.00$ & $9.00$ & $9.14$ & $20.47$ & $0.2032$ \\
% \cmidrule{1-6}

\model\ $-$ RT $-$ SH & $28.63$ &$8.06$ & $9.55$ & $23.02$ & $-0.0209$ \\
% \cmidrule{1-6}

\model\ $-$ SH & $39.77$ & $9.55$ & $8.98$ & $24.11$ & $0.1908$ \\
% \cmidrule{1-6}

\model\ $-$ PD & $36.87$ & $10.02$ & $11.22$ & $33.38$ & $0.2420$ \\
% \cmidrule{1-6}

\model\ $-$ RT & $42.01$ &$9.83$ & $16.50$ & $18.03$ & $0.2060$ \\
% \cmidrule{1-6}

\model\ $+$ DF & $39.67$ &$9.95$ & $12.69$ & $21.19$ & $0.2003$ \\
% \cmidrule{1-6}

\model\ $-$ MH-Know & $40.42$ &$10.09$ & $11.00$ & $23.97$ & $0.2429$ \\
\cdashline{1-6}
\model\ & $45.36$ & $15.71$ & $24.75$ & $25.42$ & $0.3407$ \\

\bottomrule
\end{tabular}
\caption{In the upper section of the table, we present the baseline results obtained on \data. We report  Rouge-1 (R-1), Rouge-2 (R-2), Rouge-L (R-L), Bleurt Score (BS) and QuestEval Score (QAE). In the lower section of the table, we show ablation study studying the effect of psychotherapy elements SH, PD, DF, and RT. 
% \hl{table 2 and ablation table could be merged}% Our model, \model\ yields better Rouge scores than competing baselines on R-1, R-2 and BS. We also presented a problem-specific metric, MHIC in Section \ref{mhic}.
}
%\vspace{-5mm}
\label{tab:result_and_ablation}
\end{table}


% \begin{table}[!t]\centering
% %\resizebox{\columnwidth}{!}{
% \begin{tabular}{l|rrrrr}\toprule

% % \multirow{2}{*}{Counselling Labels} &\multicolumn{5}{c}{\model\ Generated Summary } \\
% % \cmidrule{2-6}

% Counselling Label &R-1 &R-2 &R-L &QAE &BS \\
% \cmidrule{1-6}

% \model\ $-$ SH $-$ PD & $20.92$ & $5.00$ & $7.44$ & $20.71$ & $0.0019$ \\
% % \cmidrule{1-6}

% \model\ $-$ PD $-$ RT & $36.00$ & $9.00$ & $9.14$ & $20.47$ & $0.2032$ \\
% % \cmidrule{1-6}

% \model\ $-$ RT $-$ SH & $28.63$ &$8.06$ & $9.55$ & $23.02$ & $-0.0209$ \\
% % \cmidrule{1-6}

% \model\ $-$ SH & $39.77$ & $9.55$ & $8.98$ & $24.11$ & $0.1908$ \\
% % \cmidrule{1-6}

% \model\ $-$ PD & $36.87$ & $10.02$ & $11.22$ & $33.38$ & $0.2420$ \\
% % \cmidrule{1-6}

% \model\ $-$ RT & $42.01$ &$9.83$ & $16.50$ & $18.03$ & $0.2060$ \\
% % \cmidrule{1-6}

% \model\ $+$ DF & $39.67$ &$9.95$ & $12.69$ & $21.19$ & $0.2003$ \\
% % \cmidrule{1-6}

% \model\ $-$ MH-Know & $40.42$ &$10.09$ & $11.00$ & $23.97$ & $0.2429$ \\
% \cdashline{1-6}
% \model\ & $45.36$ & $15.71$ & $24.75$ & $25.42$ & $0.3407$ \\

% % \cmidrule{1-6}
% % \model\ - PD &31.44 &5.63 & 27.38 &33.55 & -0.5655 \\\cmidrule{1-6}


% % RankAE \cite{Zou_Lin_Zhao_Kang_Jiang_Sun_Zhang_Huang_Liu_2021} & 25.57 & 3.43 & 24.16 & 29.98 & -1.0631  & 24  & 6.37 & 20.15 & 30.25 & -0.7466 \\\cmidrule{1-11}

% % \textbf{\model} &\textbf{45.36} &\textbf{15.71} & 24.75 & 25.42 &\textbf{0.3407} & 7.13 & 22.12 & 17.24 &\textbf{83.21} & 0.0284 \\\midrule

% \bottomrule
% \end{tabular}
% \caption{Ablation study on the effect of different modules of \model. SH, PD, DF and RT are therapy constituents. We present our analysis on five scores to understand all aspects of summary generation.}
% \label{tab:ablation_result}
% \vspace{0mm}
% \end{table}
